The ice cone family and iterated integrals for Calabi-Yau varieties

We present for the first time fully analytic results for multi-loop equal-mass ice cone graphs in two dimensions. By analysing the leading singularities of these integrals, we find that the maximal cuts in two dimensions can be organised into two copies of the same periods that describe the Calabi-Yau varieties for the equal-mass banana integrals. We obtain a conjectural basis of master integrals at an arbitrary number of loops, and we solve the system of differential equations satisfied by the master integrals in terms of the same class of iterated integrals that have appeared earlier in the context of equal-mass banana integrals. We then go on and show that, when expressed in terms of the canonical coordinate on the moduli space, our results can naturally be written as iterated integrals involving the geometrical invariants of the Calabi-Yau varieties. Our results indicate how the concept of pure functions and transcendental weight can be extended to the case of Calabi-Yau varieties. Finally, we also obtain a novel representation of the periods of the Calabi-Yau varieties in terms of the same class of iterated integrals, and we show that the well-known quadratic relations among the periods reduce to simple shuffle relations among these iterated integrals.

==> alt_linComb.tex <==

After we have determined a basis for the master integrals of the ice cone family we still need to fix the boundary conditions. We will first explain how one can fix the boundary conditions for the master integral $I_1(s)$ which is the actual ice cone integral. Afterwards we relate this to the basis of solutions of the Gauss-Manin system \eqref{gmlloop}. \red{Mal schauen, ob ich das genau so hinbekomme.} It turns out that similarly as for the banana integrals one can find a basis of solutions with integral monodromies around all singularities and an intersection form related to the one of the banana. The master integral $I_1(s)$ will be a member of this special basis. \red{Einfach die doppelte extension, welche gute Monodromy hat und die anderen sind die vom banana welche die erste extension ist. Dadurch ist das eigentlich klar.}

For the normalization we notice that for $s=0$ the $l$-loop ice cone graph degenerates up to a normalization constant to the $l$-loop banana graph. This gives us a normalization condition for the ice cone graphs since the value of the $l$-loop banana graph at $p^2=0$ is known at least to arbitrary precision. It turns out that it is the usual $l$-loop banana integral divided by $-(l+1)$. For the first few orders we find
\begin{equation}
\begin{aligned}
	I^{(2)}_\text{Ice}(0)	&=	-\frac13\cdot I^{(2)}_\text{Ban}(0)	&&=	\frac19\left( \zeta_{1/3}(2)-\zeta_{2/3}(2)\right)	\\
	I^{(3)}_\text{Ice}(0)	&=	-\frac14\cdot I^{(3)}_\text{Ban}(0)	&&=	-\frac74\zeta(3)		\\
	I^{(4)}_\text{Ice}(0)	&=	-\frac15\cdot I^{(4)}_\text{Ban}(0)	&&= \num{7.989117602}...	\\
	I^{(5)}_\text{Ice}(0)	&=	-\frac16\cdot I^{(5)}_\text{Ban}(0)	&&= \num{-38.918052541}...
\label{normalizationcondition}
\end{aligned}
\end{equation}

For the global analytic structure of the ice cone graph we remark that the value of the ice cone integral should be a real number for small values of $s$ and that as a function of $s$ this integral is regular for small $s$. It turns out that at $s=4$ the integral exhibits a branch cut until the point at $s=\infty$. Moreover, the geometric period integral vanishing at $s=4$ is the imaginary part of the ice cone graph at infinity. This is completely analogous as for the banana integrals.

Around the point $s=\infty$ we can relate the local Frobenius basis to a basis with global integral monodromies and intersection form related to the banana one. The ice cone graph itself will be an element of this integral monodromy basis. For $l=4,5$ the requirement that the ice cone graph itself is an element in the integral monodromy basis actually gives an additional and necessary condition to determine the correct linear combination.

Let us now go through the examples for $l=2,3,4,5$ to demonstrate how this works. For the analytic continuation the apparent singularities do not play any important role. Moreover, we have checkt our results also with the results from an explicit numerical evaluation of the integral for different values of $s$ and the results agreed up to the used precision.



%=======================================
\subsubsection{The $l=2$ ice cone graph}
%=======================================

Using reduce we can find the following inhomogeneous differential equation governing the $l=2$ ice cone graph
\begin{equation}
\begin{aligned}
	&\left(	4 (-9+s) s^2+2 \left(-36+30 s-52 s^2+7 s^3\right) \theta +(-4+s) \left(18-23 s+14s^2\right) \theta ^2	\right.	\\
	&\quad	\left.	+(-4+s)^2 (9+4 s) \theta ^3	\right) I^{(2)}_\text{Ice}(s)	\\	
   	&=	2s^2 I^{(2)}_\text{Tadpole}(s)		+12I^{(2)}_\text{Bubble x Tadpole}(s)	
\label{l2iceconediff}
\end{aligned}
\end{equation}

For $|s|<\frac94$ a basis of solutions is given by
\begin{equation}
\begin{aligned}
	\omega_1		&=	\frac1{\sqrt s}\left( 1-\frac{1}{24}s+\frac{155 }{10368}s^2-\frac{1421 }{248832}s^3+\frac{53947 }{23887872}s^4\right) + \hdots 	\\
	\omega_2		&=	1+\frac{2 }{9}s+\frac{4 }{243}s^3-\frac{20 }{6561}s^4  + \hdots	\\
	\omega_3		&=	s-\frac{9 }{40}s^2+\frac{221 }{1890}s^3-\frac{3307 }{81648}s^4 + \hdots	\\
	\omega_s		&=	-\frac{7}{18}+\frac{2 }{1701}s^3-\frac{341 }{3674160}s^4	+ \hdots	~,
\label{l2omega0}
\end{aligned}
\end{equation}
such that the generic solution to \eqref{l2iceconediff} is of the form
\begin{equation}
	\omega	=	\sum_{i=1}^3 \alpha_i\omega_i	+	\omega_s	~.
\label{l2genericsol}
\end{equation}

From regularity and the normalization we can make the following ansatz for the ice cone integral
\begin{equation}
	I^{(2)}_\text{Ice}(s)	=	\left\{ \frac19\left( \zeta_{1/3}(2)-\zeta_{2/3}(2)\right)+\frac7{18}\right\}	\omega_2(s)	+	\alpha \omega_3(s)	+ \omega_s(s)	~.
\label{l2ansatz}
\end{equation}

The coefficients $\alpha$ is then determined if we require that also around $s=-9/4$ the integral is regular. From these conditions one find
\begin{equation}
	\alpha	=	-\frac{10}{81}	~.
\label{l2coeffs}
\end{equation}

Notice that the imaginary part of $I^{(2)}_\text{Ice}(s)$ at $s=\infty$ is proportional to the period that corresponds to the vanishing cycle at $s=4$ (completely similar as for the banana).

To construct the integral monodromy basis around $s=\infty$ it is convenient to rewrite the inhomogeneous differential equation in \eqref{l2iceconediff} as a homogeneous one. This gives a fifth order differential equation which has in the variable $z=1/s$ the following form
\begin{equation}
\begin{aligned}
	\mathcal L^{(2)}		&=	-8 (-1+24 z)-4 \left(10-227 z+72 z^2-60 z^3+756 z^4\right) \theta	\\
					&\quad	 -2 \left(-37+784 z-664 z^2-308 z^3+252 z^4\right) \theta ^2	\\
					&\quad	+\left(-64+1271 z-2148 z^2-1040 z^3+8568 z^4\right) \theta ^3	\\
					&\quad	+2 (-1+4 z) \left(-13+197 z+43 z^2+1008
   z^3\right) \theta ^4+(-1+4 z)^2 (4+9 z) (-1+14 z) \theta ^5
\label{l2iceconediffinfty}
\end{aligned}
\end{equation}
with $\mathcal L^{(2)}	I^{(2)}_\text{Ice}(z)=0$. A local Frobenius basis is given by
\begin{equation}
\begin{aligned}
	\tilde\omega_1		&=	\sqrt z\left( 1+\frac{7 }{8}z+\frac{339 }{128}z^2+\frac{9075 }{1024}z^3+\frac{1018563 }{32768}z^4	\right) + \hdots 	\\
	\tilde\omega_2		&=	z+\frac{17 }{10}z^3+\frac{167 }{140}z^4+\frac{919 }{90}z^5  + \hdots	\\
	\tilde\omega_3		&=	z^2+2 z^3+9 z^4+28 z^5 + \hdots	\\
	\tilde\omega_4		&=	\tilde\omega_3\log(z)	+2 z^4+6 z^5 \hdots	\\
	\tilde\omega_5		&=	\tilde\omega_3\log(z)	^2-\left(z+\frac{17 }{10}z^3-\frac{393 }{140}z^4-\frac{161 }{90}z^5\right)\log(z)	+	\frac{143 }{100}z^3+\frac{235693 }{29400}z^4+\frac{3789181}{113400} z^5 \hdots	~,
\label{l2omega0infty}
\end{aligned}
\end{equation}
which is related by the matrix
\begin{equation}
\begin{aligned}
	\left(
\begin{array}{ccccc}
 0 & 0 & 4 \pi ^2 & 0 & 0 \\
 2 \pi ^2 & 0 & 0 & 0 & 0 \\
 0 & -2 i \pi  & -\frac{11}{3}i \pi  & 4 i \pi  & 0 \\
 0 & 0 & 0 & 4 i \pi  & 0 \\
 0 & -2+i \pi  & -\frac{31}{18}+\frac{11  }{6}i \pi+\frac{2 \pi ^2}{3} & \frac{11}{6}-2 i \pi  & -1 \\
\end{array}
\right)
\label{sl2}
\end{aligned}
\end{equation}
to the integral monodromy basis. The corresponding intersection is given by
\begin{equation}
\begin{aligned}
	\left(
\begin{array}{ccccc}
 1 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 \\
\end{array}
\right)~.
\label{intersectionl2}
\end{aligned}
\end{equation}
The corresponding monodromy matrices have the following form
\begin{equation}
\begin{aligned}
	M_{s=-9/4}	&=	\left(
\begin{array}{ccccc}
 -1 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 0 & 0 \\
 -2 & 0 & 1 & 0 & 0 \\
 -2 & 0 & 0 & 1 & 0 \\
 0 & 0 & 0 & 0 & 1 \\
\end{array}
\right)	\, ,	%	
	&M_{s=0}	&=	\left(
\begin{array}{ccccc}
 0 & 1 & 0 & 0 & 0 \\
 1 & 0 & 0 & 0 & 0 \\
 0 & 0 & -1 & 0 & 0 \\
 0 & 0 & -1 & 1 & 0 \\
 0 & 0 & 0 & 0 & 1 \\
\end{array}
\right)	\\	%	
	M_{s=4}	&=	\left(
\begin{array}{ccccc}
 0 & -1 & 0 & 0 & 0 \\
 -1 & 0 & 0 & 0 & 0 \\
 0 & 0 & -1 & 0 & 0 \\
 0 & 0 & -1 & 1 & 0 \\
 0 & 0 & 1 & 0 & 1 \\
\end{array}
\right)	\, ,	%	
	&M_{s=\infty}	&=	\left(
\begin{array}{ccccc}
 1 & 0 & 0 & 0 & 0 \\
 0 & -1 & 0 & 0 & 0 \\
 -2 & 0 & 1 & 0 & 0 \\
 -2 & 0 & 0 & 1 & 0 \\
 2 & 0 & -1 & 0 & 1 \\
\end{array}
\right)	~.
\label{intmonol2}
\end{aligned}
\end{equation}



Notice that at the point $z=0$ the monodromy matrices of the banana appear as subblocks.



%=======================================
\section{The $l=3$ ice cone graph}
%=======================================

Using reduce we can find the following inhomogeneous differential equation governing the $l=3$ ice cone graph %(see \eqref{fullhigherequationinhom})
\begin{small}\begin{equation}
\begin{aligned}
	&\left\{ 12 (-4+s) s^2 \left(535552-675424 s+347256 s^2-52569 s^3+4374 s^4\right)	\right.\\
	&\quad+4 (-4+s) s \left(1548288+4658752 s-6316816 s^2+3296358 s^3-535410 s^4+45927 s^5\right) \theta 	\\
	&\quad +2 (-4+s) \left(1835008+6717440 s+7268928 s^2-14053968 s^3+7940214 s^4-1388988 s^5+124659 s^6\right) \theta^2	\\
	&\quad +(-4+s) \left(11010048-4931584 s+2122880 s^2-13895968 s^3+9008748 s^4-1710072 s^5+164025 s^6\right)
   \theta ^3		\\
   	&\quad +12 (-4+s)^2 s \left(75776+118432 s+86400 s^2-24057 s^3+4374 s^4\right) \theta ^4	\\
	&\quad\left. +(-4+s)^3   (64+9 s) \left(-14336+20576 s-5544 s^2+729 s^3\right) \theta ^5 \right\} I^{(3)}_\text{Ice}(s)	\\
	&=	6 s^2 \left(575488-287296 s+2592 s^2+6561 s^3\right) I^{(3)}_\text{Tadpole}(s) 	\\
	&\quad	+ 6 s^2 \left(-458752+345088 s-92160 s^2+6885 s^3\right) I^{(3)}_\text{Bubble x Tadpole}(s)	
\label{l3iceconediff}
\end{aligned}
\end{equation}\end{small}

For $|s|<4$ a basis of solutions is given by
\begin{equation}
\begin{aligned}
	\omega_1		&=	\frac1{\sqrt s}\left( 1+\frac{3 }{32}s+\frac{37 }{2048}s^2+\frac{59 }{16384}s^3 \right) + \hdots 	\\
	\omega_2		&=	\log(s)\omega_0	+	\frac1{\sqrt s}\left( \frac{7 }{64}s+\frac{595 }{24576}s^2+\frac{3237 }{655360}s^3 \right) + \hdots 	\\
	\omega_3		&=	1+\frac{3 }{16}s+\frac{75 }{2048}s^2+\frac{33 }{4096}s^3  + \hdots	\\
	\omega_4		&=	\log(s)\omega_3	+\frac{3571 }{204800}s^2+\frac{199951 }{60211200}s^3 + \hdots	\\
	\omega_5		&=	s+\frac{2283 }{22400}s^2+\frac{72241 }{2195200}s^3	+\hdots	\\
	\omega_s		&=	\frac{171 }{358400}s^2+\frac{39353 }{316108800}s^3	+\hdots	~,
\label{l3omega0}
\end{aligned}
\end{equation}
such that the generic solution to \eqref{l3iceconediff} is of the form
\begin{equation}
	\omega	=	\sum_{i=1}^5 \alpha_i\omega_i	+	\omega_s	~.
\label{l3genericsol}
\end{equation}

From regularity and the normalization we can make the following ansatz for the ice cone integral
\begin{equation}
	I^{(3)}_\text{Ice}(s)	=	-\frac74\zeta(3)	\omega_3(s)	+	\alpha \omega_5(s)	+	\omega_s(s)	~.
\label{l3ansatz}
\end{equation}

The coefficient $\alpha$ is then determined if we require that also around $s=-64/9$ the integral is regular. From these conditions one find
\begin{equation}
	\alpha	=	\frac1{32}	~.
\label{l3coeffs}
\end{equation}

Notice that the imaginary part of $I^{(3)}_\text{Ice}(s)$ at $s=\infty$ is proportional to the period that corresponds to the vanishing cycle at $s=4$ (completely similar as for the banana).

To construct the integral monodromy basis around $s=\infty$ it is convenient to rewrite the inhomogeneous differential equation in \eqref{l3iceconediff} as a homogeneous one. This gives a seventh order differential operator $\mathcal L^{(3)}$ \red{Shown in the appendix?}. A local Frobenius basis is given by
\begin{equation}
\begin{aligned}
	\tilde\omega_1		&=	z-\frac{4814 }{1377}z^4+\frac{5467 }{41310}z^5 + \hdots 	\\
	\tilde\omega_2		&=	z^2+\frac{1861 }{153}z^4-\frac{173833 }{9180}z^5  + \hdots	\\
	\tilde\omega_3		&=	z^3-\frac{25 }{153}z^4+\frac{164653 }{9180}z^5 + \hdots	\\
	\tilde\omega_4		&=	(\tilde\omega_1+\frac{86}{27}\tilde\omega_3)\log(z)	-\frac{478007 }{37179}z^4+\frac{35276429 }{2230740}z^5 \hdots	\\
	\tilde\omega_5		&=	(\tilde\omega_2+\tilde\omega_3)\log(z)	+\frac{1021 }{153}z^4-\frac{44957}{4590}  z^5\hdots	\\
	\tilde\omega_6		&=	(\tilde\omega_2+\tilde\omega_3)\log(z)^2	+\left(-4 z^3+14 z^4-\frac{274 }{3}z^5\right)\log(z)	-\frac{53}{306}z^4-\frac{41654 }{2295}z^5	 \hdots	\\
	\tilde\omega_7		&=	(\tilde\omega_2+\tilde\omega_3)\log(z)^3	+\left(-6 z^3+21 z^4\right)\log(z)^2	+\left(\frac{409 }{54}z^3-\frac{427 }{243}z^4\right)\log(z)	-\frac{294139 }{74358}z^4 \hdots	~,
\label{ltomega0infty}
\end{aligned}
\end{equation}
which is related by the matrix \red{To long expression. In appendix???}
%\begin{equation}
%\begin{aligned}
%	\left(
%\begin{array}{ccccc}
% 0 & 0 & 4 \pi ^2 & 0 & 0 \\
% 2 \pi ^2 & 0 & 0 & 0 & 0 \\
% 0 & -2 i \pi  & -\frac{1}{3} (11 i \pi ) & 4 i \pi  & 0 \\
% 0 & 0 & 0 & 4 i \pi  & 0 \\
% 0 & -2+i \pi  & -\frac{31}{18}+\frac{11 i \pi }{6}+\frac{2 \pi ^2}{3} & \frac{11}{6}-2 i \pi  & -1 \\
%\end{array}
%\right)
%\label{sl3}
%\end{aligned}
%\end{equation}
to the integral monodromy basis. The corresponding intersection is given by
\begin{equation}
\begin{aligned}
	\left(
\begin{array}{ccccccc}
 0 & 1 & 0 & 0 & 0 & 0 & 0 \\
 -1 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 1 & 0 & 0 & 0 \\
 0 & 0 & -1 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\end{array}
\right)~.
\label{intersectionl3}
\end{aligned}
\end{equation}
The corresponding monodromy matrices have the following form
\begin{equation}
\begin{aligned}
	M_{s=-64/9}	&=	\left(
\begin{array}{ccccccc}
 -5 & -6 & 0 & 0 & 0 & 0 & 0 \\
 6 & 7 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 1 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 1 & 0 & 0 & 0 \\
 1 & 1 & 0 & 0 & 1 & 0 & 0 \\
 36 & 36 & 0 & 0 & 0 & 1 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
\end{array}
\right)	\, ,	%	
	&M_{s=0}	&=	\left(
\begin{array}{ccccccc}
 0 & 0 & 5 & -6 & 0 & 0 & 0 \\
 0 & 0 & -4 & 5 & 0 & 0 & 0 \\
 -7 & -12 & 0 & 0 & 0 & 0 & 0 \\
 -4 & -7 & 0 & 0 & 0 & 0 & 0 \\
 -1 & -1 & -1 & 1 & -1 & 0 & 0 \\
 1 & 0 & -37 & 48 & -12 & 1 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
\end{array}
\right)	\\	%	
	M_{s=4}	&=	\left(
\begin{array}{ccccccc}
 0 & 0 & -1 & 0 & 0 & 0 & 0 \\
 0 & 0 & 1 & -1 & 0 & 0 & 0 \\
 -1 & 0 & 0 & 0 & 0 & 0 & 0 \\
 -1 & -1 & 0 & 0 & 0 & 0 & 0 \\
 -1 & -1 & 0 & 1 & -1 & 0 & 0 \\
 7 & 12 & -5 & 24 & -12 & 1 & 0 \\
 6 & 6 & 0 & 0 & 6 & 0 & 1 \\
\end{array}
\right)	\, ,	%	
	&M_{s=\infty}	&=	\left(
\begin{array}{ccccccc}
 1 & 0 & 0 & 0 & 0 & 0 & 0 \\
 1 & 1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 7 & -12 & 0 & 0 & 0 \\
 0 & 0 & 3 & -5 & 0 & 0 & 0 \\
 -2 & -1 & 0 & 0 & 1 & 0 & 0 \\
 -20 & -12 & 6 & -12 & 0 & 1 & 0 \\
 0 & 0 & 0 & 0 & -6 & 0 & 1 \\
\end{array}
\right)	~.
\label{intmonol3}
\end{aligned}
\end{equation}



Notice that at the point $z=0$ the monodromy matrices of the two-loop banana appear as subblocks.


















%=======================================
\section{The $l=4$ ice cone graph}
%=======================================

Using reduce we can find the following inhomogeneous differential equation governing the $l=4$ ice cone graph (the precise form of $\mathcal L^{(7)}$ is to long to be presented here)
\begin{small}\begin{equation}
\begin{aligned}
	& \mathcal L^{(7)}  I^{(4)}_\text{Ice}(s)	\\
	&=	48 s^3 \left(1565093745000-3790284451200 s+2552366859732 s^2-750006988659 s^3+85444508880
   s^4	\right.	\\
   	&\quad	\left.-273384864 s^5-91287552 s^6+8388608 s^7\right) I^{(4)}_\text{Tadpole}(s) 	\\
	&\quad	-48 s^3 \left(1565093745000-332227388700 s-150609447738 s^2-122742859221 s^3+61139437632
   s^4	\right.	\\
   	&\quad	\left. -7411916880 s^5+317910528 s^6+4046848 s^7\right) I^{(4)}_\text{Bubble x Tadpole}(s)	
\label{l4iceconediff}
\end{aligned}
\end{equation}\end{small}

For $|s|<4$ a basis of solutions is given by
\begin{equation}
\begin{aligned}
	\omega_1		&=	\frac1{\sqrt s}\left( 1-\frac{159977 }{155520000}s^3-\frac{51013073 }{2612736000000}s^4-\frac{64391897063}{783820800000000}s^5 \right) + \hdots 	\\
	\omega_2		&=	\sqrt s	\left(	1+\frac{308281 }{6480000}s^2-\frac{6338401 }{1944000000}s^3+\frac{237187643153 }{65318400000000}s^4-\frac{6291221336161 }{9797760000000000}s^5 \right) + \hdots 	\\
	\omega_3		&=	s^{3/2}\left	(	1+\frac{1}{360}s+\frac{367 }{5760}s^2-\frac{27457 }{5225472}s^3+\frac{41341529}{7524679680}s^4-\frac{427712531 }{397303087104}s^5	\right) + \hdots	\\
	\omega_4		&=	1-\frac{5 }{27702}s^4+\frac{84397 }{15997905000}s^5 + \hdots	\\
	\omega_5		&=	s-\frac{16147 }{8015112}s^4-\frac{207893251 }{661246740000}s^5	+\hdots	\\
	\omega_6		&=	s^2+\frac{80677 }{1113210}s^4-\frac{118989119 }{18367965000}s^5	+\hdots	\\
	\omega_7		&=	s^3-\frac{5525 }{127224}s^4+\frac{687547603 }{7871985000}s^5	+\hdots	\\
	\omega_s		&=	-\frac{3149 }{150283350}s^4-\frac{8630999 }{14878051650000}s^5	+\hdots	~,
\label{l2omega0}
\end{aligned}
\end{equation}
such that the generic solution to \eqref{l4iceconediff} is of the form
\begin{equation}
	\omega	=	\sum_{i=1}^7 \alpha_i\omega_i	+	\omega_s	~.
\label{l3genericsol}
\end{equation}

From regularity and the normalization we can make the following ansatz for the ice cone integral
\begin{equation}
	I^{(4)}_\text{Ice}(s)	=	-\frac15\cdot I^{(4)}_\text{Ban}(0)	\omega_4(s)	+	\alpha \omega_5(s)	+\beta\omega_6(s)	+\gamma\omega_7(s)	+\omega_s(s)	~.
\label{l2ansatz}
\end{equation}

The coefficient $\alpha,\beta$ and $\gamma$ are then determined if we require that also around $s=-225/16$ and $s=-9/4$ the integral is regular and that the integral is an element of the integral monodromy basis. From these conditions one find
\begin{equation}
	\alpha	=	\num{1.360989211}...	~,	\quad \beta=\num{0.273625981}...	\quad\text{and}\quad		\gamma=	\num{0.058762373}... 	~.
\label{l2coeffs}
\end{equation}

Notice that the imaginary part of $I^{(4)}_\text{Ice}(s)$ at $s=\infty$ is proportional to the period that corresponds to the vanishing cycle at $s=4$ (completely similar as for the banana).

\red{Relation to integral monodromy basis is quite long. Where can we put it? Mathematica file?}


%=======================================
\section{The $l=5$ ice cone graph}
%=======================================

Using reduce we can find the following inhomogeneous differential equation governing the $l=5$ ice cone graph (the precise form of $\mathcal L^{(9)}$ is to long to be presented here)
\begin{footnotesize}\begin{equation}
\begin{aligned}
	& \mathcal L^{(9)}  I^{(5)}_\text{Ice}(s)	\\
	&=	120 s^3 \left(1323003960610665372057600+46545441088168543641403392s-37115693176052021968502784 s^2	\right.	\\
   	&\quad	-1870130656371384476762112s^3+16846559972963032620466176s^4	-3491291001903503033606144s^5	\\
   	&\quad-576149516620876317328896 s^6	+211232961302138587771200 s^7-35208906037161866595000s^8	\\
   	&\quad	\left. +3160146690254520140625 s^9-7004990052928125000 s^{10} +15177630498046875s^{11}\right)	I^{(4)}_\text{Tadpole}(s) 	\\[1ex]
	&\quad	+120 s^3 \left(-1323003960610665372057600-9678083295903431692124160s+7077581271464450495348736 s^2\right.	\\
   	&\quad	-11504293228388998170279936s^3-4103825008809334022995968 s^4+5843328878864356744929280s^5	\\
   	&\quad	-1729353815427759467687424 s^6+166808195785015717176000 s^7-1429438291120807371000s^8	\\
   	&\quad	\left.+1436858394364265625 s^9+43973526493125000 s^{10}\right)	I^{(4)}_\text{Bubble x Tadpole}(s)	
\label{l5iceconediff}
\end{aligned}
\end{equation}\end{footnotesize}

For $|s|<4$ a basis of solutions is given by
\begin{equation}
\begin{aligned}
	\omega_1		&=	\frac1{\sqrt s}\left( 1-\frac{32021 }{99532800}s^3-\frac{15619817 }{214035333120}s^4-\frac{136846740221
   }{6934744793088000}s^5 \right) + \hdots 	\\
	\omega_2		&=	\sqrt s	\left(	1+\frac{96583 }{12441600}s^2+\frac{127234537 }{187280916480}s^3+\frac{1174273371181
   }{6067901693952000}s^4 \right) + \hdots 	\\
	\omega_3		&=	s^{3/2}\left	(	1+\frac{29 }{160}s+\frac{81 }{1792}s^2+\frac{23171 }{2293760}s^3	\right) + \hdots	\\
	\omega_4		&=	\log(s)\omega_3+s^{3/2}\left(	\frac{6299 }{259200}s+\frac{1740605 }{390168576}s^2	\right) + \hdots	\\
	\omega_5		&=	1+\frac{5}{32}s+\frac{333}{10240}s^2+\frac{373}{53760}s^3+\frac{39055}{25165824}s^4+\frac{36467491}{103347650560}s^5 + \hdots	\\
	\omega_6		&=	s-\frac{114822387163 }{59156407296000}s^4-\frac{955978061039 }{1735254614016000}s^5	+\hdots	\\
	\omega_7		&=	s^2+\frac{124928319127 }{17746922188800}s^4-\frac{14125076390449 }{14576138757734400}s^5	+\hdots	\\
	\omega_8		&=	s^3+\frac{8420329873 }{35212147200}s^4+\frac{997738894687 }{14460455116800}s^5	+\hdots	\\
	\omega_9		&=	\log(s)\omega_5 -\frac{141378181900339}{15265192589918208000}s^4-\frac{799878948199233611}{275831853304762073088000}s^5	+\hdots	\\
	\omega_s		&=	-\frac{3810027709}{283950755020800}s^4-\frac{3030002057743}{699654660371251200}s^5	+\hdots	~,
\label{l5omega0}
\end{aligned}
\end{equation}
such that the generic solution to \eqref{l5iceconediff} is of the form
\begin{equation}
	\omega	=	\sum_{i=1}^9 \alpha_i\omega_i	+	\omega_s	~.
\label{l3genericsol}
\end{equation}

From regularity and the normalization we can make the following ansatz for the ice cone integral
\begin{equation}
	I^{(5)}_\text{Ice}(s)	=	-\frac16\cdot I^{(5)}_\text{Ban}(0)	\omega_5(s)	+	\alpha \omega_6(s)	+\beta\omega_7(s)	+\gamma\omega_8(s)	+\omega_s(s)	~.
\label{l2ansatz}
\end{equation}

The coefficient $\alpha,\beta$ and $\gamma$ are then determined if we require that also around $s=-576/25$ and $s=-64/9$ the integral is regular and that the integral is an element of the integral monodromy basis. From these conditions one find
\begin{equation}
	\alpha	=	\num{-0.489610975}...	~,	\quad \beta=\num{-0.051948475}...	\quad\text{and}\quad		\gamma=	\num{-0.01259811}... 	~.
\label{l2coeffs}
\end{equation}

\red{Relation to integral monodromy basis is quite long. Where can we put it? Mathematica file?}
